NLPBench: Evaluating Large Language Models on Solving NLP Problems

Recent developments in large language models (LLMs) have shown promise in enhancing the capabilities of natural language processing (NLP). Despite these successes, there remains a dearth of research dedicated to the NLP problem-solving abilities of LLMs. To fill the gap in this area, we present a unique benchmarking dataset, NLPBench, comprising 378 college-level NLP questions spanning various NLP topics sourced from Yale University's prior final exams. NLPBench includes questions with context, in which multiple sub-questions share the same public information, and diverse question types, including multiple choice, short answer, and math. Our evaluation, centered on LLMs such as GPT-3.5/4, PaLM-2, and LLAMA-2, incorporates advanced prompting strategies like the chain-of-thought (CoT) and tree-of-thought (ToT). Our study reveals that the effectiveness of the advanced prompting strategies can be inconsistent, occasionally damaging LLM performance, especially in smaller models like the LLAMA-2 (13b). Furthermore, our manual assessment illuminated specific shortcomings in LLMs' scientific problem-solving skills, with weaknesses in logical decomposition and reasoning notably affecting results.

==> tables/categories.tex <==
\begin{table}[h]
\centering
\caption{Experimental results in terms of accuracy (\%) on our proposed dataset. The best average scores in each type of question are highlighted in \best{bold}, and the best average scores for each model in a specific type of question are \secbest{underlined}.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccccccccccccccccccc@{}}
\toprule
\multirow{2}{*}{Model} &
  \multirow{2}{*}{Setting} &
  \multicolumn{7}{c}{Multiple Choice} &
  \multicolumn{7}{c}{Short Answer} &
  \multicolumn{7}{c}{Math} \\ 
  \cmidrule(l){3-9} 
  \cmidrule(l){10-16}
  \cmidrule(l){17-23}
 &
   &
  \acronym{lmsp} &
  \acronym{sl} &
  \acronym{pdda} &
  \acronym{irtm} &
  \acronym{ai} &
  \acronym{ot} &
  Avg. &
  \acronym{lmsp} &
  \acronym{sl} &
  \acronym{pdda} &
  \acronym{irtm} &
  \acronym{ai} &
  \acronym{ot} &
  Avg. &
  \acronym{lmsp} &
  \acronym{sl} &
  \acronym{pdda} &
  \acronym{irtm} &
  \acronym{ai} &
  \acronym{ot} &
  Avg. \\ \midrule
\multirow{10}{*}{GPT-3.5} &
  ZS &
  47.83 &
  62.50 &
  100.00 &
  58.82 &
  35.48 &
  60.00 &
  50.64 &
  71.26 &
  70.27 &
  52.78 &
  66.67 &
  68.83 &
  78.43 &
  \secbest{69.99} &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+SYS &
  44.12 &
  40.63 &
  0.0 &
  35.29 &
  38.71 &
  50.00 &
  41.51 &
  66.67 &
  64.86 &
  58.33 &
  33.33 &
  87.88 &
  70.59 &
  68.75 &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+CoT &
  49.28 &
  62.50 &
  50.00 &
  41.18 &
  48.39 &
  80.00 &
  \secbest{52.83} &
  54.02 &
  64.86 &
  52.78 &
  50.00 &
  53.68 &
  35.29 &
  54.19 &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+CoT+SYS &
  38.24 &
  40.62 &
  100.00 &
  35.29 &
  48.39 &
  30.00 &
  40.25 &
  65.52 &
  51.35 &
  50.00 &
  50.00 &
  84.85 &
  64.71 &
  64.58 &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+ToT &
  30.88 &
  21.88 &
  100.00 &
  23.53 &
  32.26 &
  20.00 &
  28.30 &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS &
  33.82 &
  46.88 &
  100.00 &
  29.41 &
  41.94 &
  40.00 &
  38.36 &
  71.26 &
  54.05 &
  16.67 &
  66.67 &
  84.85 &
  58.82 &
  65.63 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+SYS &
  45.59 &
  46.88 &
  100.00 &
  35.29 &
  45.16 &
  40.00 &
  44.65 &
  66.67 &
  54.05 &
  25.00 &
  66.67 &
  78.79 &
  52.94 &
  62.50 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+CoT &
  42.65 &
  43.75 &
  100.00 &
  29.41 &
  38.71 &
  30.00 &
  40.25 &
  65.52 &
  59.46 &
  50.00 &
  50.00 &
  69.70 &
  70.59 &
  64.06 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+SYS+CoT &
  41.17 &
  50.00 &
  100.00 &
  52.94 &
  41.93 &
  60.00 &
  45.91 &
  66.66 &
  64.86 &
  25.00 &
  66.67 &
  75.76 &
  70.59 &
  65.63 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+ToT &
  33.82 &
  25.00 &
  0.00 &
  29.41 &
  16.12 &
  30.00 &
  27.67 &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
   &
   &
   &
   &
   &
   &
   \\ \midrule
\multirow{10}{*}{GPT-4} &
  ZS &
  62.32 &
  78.12 &
  50.00 &
  82.35 &
  74.19 &
  100.00 &
  72.25 &
  75.86 &
  75.68 &
  52.78 &
  83.33 &
  85.28 &
  66.67 &
  75.42 &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+SYS &
  57.35 &
  56.25 &
  100.00 &
  58.82 &
  77.42 &
  40.00 &
  60.38 &
  82.76 &
  75.68 &
  75.00 &
  100.00 &
  87.88 &
  82.35 &
  \best{\secbest{82.29}} &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+CoT &
  68.12 &
  75.00 &
  50.00 &
  82.35 &
  74.19 &
  100.00 &
  \best{\secbest{74.10}} &
  70.11 &
  59.46 &
  44.44 &
  100.00 &
  76.19 &
  72.55 &
  68.65 &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+CoT+SYS &
  55.88 &
  62.50 &
  100.00 &
  52.94 &
  64.52 &
  60.00 &
  59.12 &
  78.16 &
  67.57 &
  41.67 &
  66.67 &
  84.85 &
  70.59 &
  73.95 &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+ToT &
  58.82 &
  50.00 &
  100.00 &
  58.82 &
  38.71 &
  80.00 &
  54.72 &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS &
  66.18 &
  62.50 &
  100.00 &
  64.71 &
  64.52 &
  60.00 &
  64.78 &
  81.61 &
  67.57 &
  58.33 &
  83.33 &
  81.82 &
  76.47 &
  77.08 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+SYS &
  61.76 &
  56.25 &
  100.00 &
  70.59 &
  61.29 &
  60.00 &
  61.64 &
  86.21 &
  67.57 &
  50.00 &
  83.33 &
  93.94 &
  76.47 &
  80.73 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+CoT &
  61.76 &
  62.50 &
  100.00 &
  64.71 &
  64.51 &
  60.00 &
  62.89 &
  85.06 &
  59.46 &
  50.00 &
  100.00 &
  87.88 &
  70.59 &
  77.60 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+SYS+CoT &
  60.29 &
  59.38 &
  100.00 &
  64.71 &
  67.74 &
  70.00 &
  62.89 &
  83.91 &
  72.97 &
  58.33 &
  100.00 &
  81.82 &
  58.82 &
  78.13 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+ToT &
  57.35 &
  56.25 &
  100.00 &
  58.82 &
  41.94 &
  60.00 &
  54.72 &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
   &
   &
   &
   &
   &
   &
   \\ \midrule
\multirow{10}{*}{PaLM 2} &
  ZS &
  33.82 &
  40.63 &
  100.00 &
  35.29 &
  51.61 &
  50.00 &
  40.25 &
  39.08 &
  48.65 &
  33.33 &
  50.00 &
  60.61 &
  41.18 &
  44.79 &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+SYS &
  45.59 &
  43.75 &
  100.00 &
  47.06 &
  54.84 &
  50.00 &
  \secbest{47.80} &
  45.98 &
  45.95 &
  41.67 &
  33.33 &
  57.58 &
  41.18 &
  46.88 &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+CoT &
  33.82 &
  40.63 &
  100.00 &
  35.29 &
  48.39 &
  40.00 &
  38.99 &
  44.83 &
  45.94 &
  33.33 &
  50.00 &
  51.52 &
  29.41 &
  44.27 &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+CoT+SYS &
  38.23 &
  46.88 &
  100.00 &
  47.06 &
  41.94 &
  50.00 &
  42.77 &
  35.63 &
  32.43 &
  25.00 &
  66.67 &
  45.46 &
  35.29 &
  36.98 &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+ToT &
  5.88 &
  3.12 &
  0.00 &
  0.00 &
  6.45 &
  0.00 &
  4.40 &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS &
  30.88 &
  46.88 &
  100.00 &
  41.18 &
  48.38 &
  50.00 &
  40.25 &
  43.68 &
  54.05 &
  50.00 &
  66.67 &
  60.61 &
  47.06 &
  \secbest{50.00} &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+SYS &
  33.82 &
  40.63 &
  100.00 &
  52.94 &
  45.16 &
  50.00 &
  40.88 &
  42.53 &
  51.35 &
  25.00 &
  50.00 &
  57.58 &
  41.18 &
  45.83 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+CoT &
  38.24 &
  43.75 &
  100.00 &
  52.94 &
  38.71 &
  40.00 &
  41.51 &
  42.53 &
  51.35 &
  25.00 &
  50.00 &
  57.58 &
  41.18 &
  45.83 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+SYS+CoT &
  35.29 &
  40.63 &
  100.00 &
  41.18 &
  38.71 &
  50.00 &
  38.99 &
  45.98 &
  51.35 &
  41.67 &
  66.67 &
  63.64 &
  35.29 &
  49.48 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+ToT &
  11.76 &
  6.25 &
  0.00 &
  5.88 &
  12.90 &
  0.00 &
  9.43 &
  - &
  - &
  - &
  - &
  - &
  - &
  - &
   &
   &
   &
   &
   &
   &
   \\ \midrule\midrule
\multirow{8}{*}{LLAMA 2-13b} &
  ZS &
  16.18 &
  28.13 &
  0.00 &
  29.41 &
  16.13 &
  30.00 &
  20.75 &
  37.93 &
  51.35 &
  16.67 &
  66.67 &
  36.36 &
  23.53 &
  \secbest{38.54} &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+SYS &
  33.82 &
  40.63 &
  0.00 &
  35.29 &
  22.58 &
  40.00 &
  33.33 &
  37.93 &
  37.83 &
  25.00 &
  66.67 &
  48.48 &
  23.53 &
  \secbest{38.54} &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+CoT &
  22.06 &
  15.63 &
  0.00 &
  11.76 &
  25.81 &
  20.00 &
  20.13 &
  12.64 &
  27.03 &
  8.33 &
  33.33 &
  27.27 &
  11.76 &
  18.23 &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+CoT+SYS &
  22.06 &
  37.50 &
  0.00 &
  29.41 &
  39.03 &
  30.00 &
  27.67 &
  19.54 &
  18.92 &
  8.33 &
  16.67 &
  24.24 &
  11.76 &
  18.75 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS &
  26.47 &
  37.50 &
  100.00 &
  29.41 &
  16.13 &
  40.00 &
  28.30 &
  14.94 &
  5.41 &
  8.33 &
  0.00 &
  6.06 &
  0.00 &
  9.38 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+SYS &
  33.82 &
  46.88 &
  100.00 &
  29.41 &
  22.58 &
  40.00 &
  \secbest{34.59} &
  13.79 &
  8.11 &
  8.33 &
  16.67 &
  6.06 &
  0.00 &
  9.90 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+CoT &
  23.53 &
  43.75 &
  0.00 &
  29.41 &
  16.13 &
  40.00 &
  27.67 &
  16.09 &
  5.41 &
  16.67 &
  16.67 &
  3.03 &
  0.00 &
  10.42 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+SYS+CoT &
  36.76 &
  40.63 &
  100.00 &
  29.41 &
  16.13 &
  40.00 &
  33.33 &
  1.49 &
  8.11 &
  16.67 &
  16.67 &
  9.09 &
  0.00 &
  11.46 &
   &
   &
   &
   &
   &
   &
   \\ \midrule
\multirow{8}{*}{LLAMA 2-70b} &
  ZS &
  22.06 &
  21.88 &
  0.00 &
  11.76 &
  35.48 &
  30.00 &
  23.90 &
  51.72 &
  43.24 &
  16.67 &
  50.00 &
  57.58 &
  52.94 &
  48.96 &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+SYS &
  25.00 &
  21.88 &
  100.00 &
  17.65 &
  38.71 &
  0.00 &
  25.16 &
  57.47 &
  51.35 &
  25.00 &
  33.33 &
  57.58 &
  41.18 &
  \secbest{52.08} &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+CoT &
  11.76 &
  28.13 &
  0.00 &
  11.76 &
  35.48 &
  60.00 &
  22.64 &
  19.54 &
  40.54 &
  0.00 &
  50.00 &
  36.36 &
  17.65 &
  26.04 &
   &
   &
   &
   &
   &
   &
   \\
 &
  ZS+CoT+SYS &
  39.71 &
  34.38 &
  100.00 &
  41.18 &
  32.26 &
  50.00 &
  \secbest{38.36} &
  29.88 &
  35.14 &
  16.67 &
  33.33 &
  39.39 &
  17.65 &
  30.73 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS &
  20.59 &
  40.63 &
  100.00 &
  23.53 &
  32.26 &
  50.00 &
  29.56 &
  44.83 &
  43.24 &
  25.00 &
  66.67 &
  60.61 &
  29.41 &
  45.31 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+SYS &
  33.82 &
  37.50 &
  100.00 &
  17.65 &
  32.26 &
  50.00 &
  33.96 &
  44.82 &
  43.24 &
  33.33 &
  66.67 &
  51.52 &
  35.29 &
  44.79 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+CoT &
  27.94 &
  43.75 &
  100.00 &
  29.41 &
  22.58 &
  40.00 &
  31.45 &
  44.83 &
  37.84 &
  33.33 &
  33.33 &
  39.40 &
  58.82 &
  42.71 &
   &
   &
   &
   &
   &
   &
   \\
 &
  FS+SYS+CoT &
  42.65 &
  34.38 &
  100.00 &
  23.53 &
  25.81 &
  60.00 &
  37.11 &
  48.28 &
  24.32 &
  33.33 &
  50.00 &
  39.40 &
  29.41 &
  39.58 &
   &
   &
   &
   &
   &
   &
   \\  \bottomrule
\end{tabular}%
}
\end{table}
